am-AMM: An Auction-Managed Automated Market Maker

Automated market makers (AMMs) have emerged as the dominant market mechanism for trading on decentralized exchanges implemented on blockchains. This paper presents a single mechanism that targets two important unsolved problems for AMMs: reducing losses to informed orderflow, and maximizing revenue from uninformed orderflow. The ``auction-managed AMM'' works by running a censorship-resistant onchain auction for the right to temporarily act as ``pool manager'' for a constant-product AMM. The pool manager sets the swap fee rate on the pool, and also receives the accrued fees from swaps. The pool manager can exclusively capture some arbitrage by trading against the pool in response to small price movements, and also can set swap fees incorporating price sensitivity of retail orderflow and adapting to changing market conditions, with the benefits from both ultimately accruing to liquidity providers. Liquidity providers can enter and exit the pool freely in response to changing rent, though they must pay a small fee on withdrawal. We prove that under certain assumptions, this AMM should have higher liquidity in equilibrium than any standard, fixed-fee AMM.

==> other_discussion.tex <==

\paraheader{Censorship}

The Harberger lease attempts to solve the short-term censorship issues noted in \citet{pai2023censorship}. While blockchains support liveness (the guaranteed \textbf{eventual} inclusion of transactions), adversarial actors can impact short-term inclusion of specific transactions. This is particularly detrimental to time-sensitive financial markets. There are two important forms of censorship for the fee-auction AMM - \textit{bid censorship} and \textit{MEV censorship}. 

Bid censorship is when a block proposer does not include any valid bids larger than the current bid, which artificially lowers the market price. The continuous structure of the Harberger lease auction means that bids can effectively be placed for blocks arbitrarily far in the future. This reduces the power of individual proposers to.

MEV censoring is when a block proposer censors any transaction that would create MEV for the current fee manager. Adversarial actors are incentivized to censor the valuable transactions and only include them at the block in which they become the fee manager. To mitigate this type of censorship, we enforce a delay of $K$ blocks between the usurpation of fee managers. The longer the delay, the more difficult it is to censor these MEV transactions as they must be censored until the adversary becomes the fee manager. 

These two mechanisms are at odds with each other. The block delay slows down price discovery but mitigates MEV censorship. The continuous time auction improves price discovery, but creates more opportunities for MEV censoring by allowing the fee managers to update more frequently. However, correctly parameterizing the block delay and minimum bid epoch, the auction can accurately reflect market prices while mitigating both bid and MEV censorship.


\paraheader{AMM Structure}

In addition to enforcing the auction mechanism described above, the AMM enforces a few properties on the underlying pool. It is responsible for setting the dynamic fee on the pool, maintaining consistent wide-range liquidity (as needed for building on top of a CLMM), setting appropriate withdrawal fees for LPs, and collecting and distributing funds between the transacting participants - the managers and the pool LPs.  

First, the AMM allows setting dynamic fees by continually updating fee setting permissions to the new manager at each auction turnover. While the manager may decide to change the fee at any time, it will not update the core pool state until the block following the update transaction. This ensures that the manager, who could also be the block proposer, cannot determine the next state of the chain at the same block that the fee adjustment can be made on the pool. This minimizes the risk of block proposers monopolizing the manager permissions  and requires that some risk is taken by the manager. To avoid other possible griefs by managers, the AMM also enforces a max fee of 1\%.

The AMM must also allocate the auction rent and swap fees to the appropriate parties. When a new fee manager is determined, the manager puts down a deposit of at least 1 epoch’s worth of rent. The rent is distributed to all LPs as they are always in-range on a CPMM and will always accrue the rent as fees weighted according to the underlying liquidity amount. In return, the manager receives all underlying swap fees for as long as they hold the winning bid. The fees are first accrued to the contract itself, and then distributed to the correct manager.

LPs should not be able to evade short term price risk by removing and subsequently redepositing underlying liquidity. Instead of enforcing liquidity locks for LPs, the AMM imposes a relatively small withdrawal fee taken on the underlying burn amount. In the short term, LPs must be indifferent to withdrawing, and bearing a withdrawal fee or maintaining their position, and bearing arbitrage loss. Thus, the expected loss from the withdrawal fee should approximately equal the expected loss from a one block arbitrage. More details about this can be found in the appendix.

